Comparative Analysis of Zero-Shot Capability of Time-Series Foundation Models in Short-Term Load Prediction

Short-term load prediction (STLP) is critical for modern power distribution system operations, particularly as demand and generation uncertainties grow with the integration of low-carbon technologies, such as electric vehicles and photovoltaics. In this study, we evaluate the zero-shot prediction capabilities of five Time-Series Foundation Models (TSFMs)-a new approach for STLP where models perform predictions without task-specific training-against two classical models, Gaussian Process (GP) and Support Vector Regression (SVR), which are trained on task-specific datasets. Our findings indicate that even without training, TSFMs like Chronos, TimesFM, and TimeGPT can surpass the performance of GP and SVR. This finding highlights the potential of TSFMs in STLP.

==> can.tex <==

\onecolumn
\begin{longtable}{ccccccccc}
\caption{Results of the Experiments.}\\
\hline
\textbf{Country} & \textbf{Type} & \textbf{Resolution} & \textbf{Model} & \textbf{Q 10\%} & \textbf{Q 50\%} & \textbf{Q 90\%} &\textbf{ MAE} & \textbf{RMSE} \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : GE-A-15}} \\
\hline
GE & Agg & 15m & Lag-llama & 0.291464 & 0.606402 & 0.529585 & 1.212804 & 1.852752 \\
GE & Agg & 15m & GP & 0.222046 & 0.680172 & 0.602423 & 1.360344 & 2.203794 \\
GE & Agg & 15m & SVR & / & / & / & 1.053772 & 1.619547 \\
GE & Agg & 15m & TimesFM & / & / & / & 1.174719 & 1.808168 \\
GE & Agg & 15m & TimeGPT & / & / & / & 1.134850 & 1.630999 \\
GE & Agg & 15m & Chronos-small & \underline{0.108502} & \underline{0.255215} & \underline{0.183157} & \underline{0.510431} & \underline{0.897094} \\
GE & Agg & 15m & Moment & / & / & / & 1.327071 & 1.705115 \\
GE & Agg & 15m & Chronos-tiny & 0.240727 & 0.456293 & 0.251467 & 0.912586 & 1.472509 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : GE-A-30}} \\
\hline

GE & Agg & 30m & Lag-llama & 0.496286 & 1.040308 & 0.772933 & 2.080616 & 3.208916 \\
GE & Agg & 30m & GP & 0.435174 & 1.351805 & 1.236134 & 2.703610 & 4.371987 \\
GE & Agg & 30m & SVR & / & / & / & 2.105799 & 3.247641 \\
GE & Agg & 30m & TimesFM & / & / & / & 1.312574 & 2.092836 \\
GE & Agg & 30m & TimeGPT & / & / & / & 2.174604 & 3.034611 \\
GE & Agg & 30m & Chronos-small & 0.400197 & \underline{0.624696} & \underline{0.437710} & \underline{1.249392} & \underline{2.125837} \\
GE & Agg & 30m & Moment & / & / & / & 2.760869 & 3.470382 \\
GE & Agg & 30m & Chronos-tiny & \underline{0.311118} & 0.668856 & 0.504947 & 1.337712 & 2.259838 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : GE-A-60}} \\
\hline

GE & Agg & 60m & Lag-llama & 0.685352 & 2.032657 & 1.691593 & 4.065313 & 6.168018 \\
GE & Agg & 60m & GP & 0.868131 & 2.700515 & 2.444953 & 5.401030 & 8.749636 \\
GE & Agg & 60m & SVR & / & / & / & 4.221373 & 6.479941 \\
GE & Agg & 60m & TimesFM & / & / & / & 2.106448 & 3.756486 \\
GE & Agg & 60m & TimeGPT & / & / & / & 2.068576 & \underline{3.285496} \\
GE & Agg & 60m & Chronos-small & \underline{0.581339} & 0.928824 & \underline{0.531181} & 1.857647 & 3.373604 \\
GE & Agg & 60m & Moment & / & / & / & 5.313778 & 6.735971 \\
GE & Agg & 60m & Chronos-tiny & 0.609318 & \underline{0.905072} & 0.480884 & \underline{1.810143} & 3.323062 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : GE-I-15}} \\
\hline

GE & Ind & 15m & Lag-llama & 0.052957 & 0.142462 & 0.128637 & 0.284924 & 0.476902 \\
GE & Ind & 15m & GP & 0.033509 & 0.092915 & 0.079206 & 0.185830 & 0.349711 \\
GE & Ind & 15m & SVR & / & / & / & 0.206299 & 0.342876 \\
GE & Ind & 15m & TimesFM & / & / & / & \underline{0.077992} & \underline{0.240639} \\
GE & Ind & 15m & TimeGPT & / & / & / & 0.220186 & 0.329946 \\
GE & Ind & 15m & Chronos-small & 0.026315 & \underline{0.066404} & \underline{0.067654} & 0.132808 & 0.270109 \\
GE & Ind & 15m & Moment & / & / & / & 0.275583 & 0.411651 \\
GE & Ind & 15m & Chronos-tiny & \underline{0.024545} & 0.087524 & 0.101449 & 0.175048 & 0.356585 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : GE-I-30}} \\
\hline

GE & Ind & 30m & Lag-llama & 0.081176 & 0.235791 & 0.232103 & 0.471582 & 0.835188 \\
GE & Ind & 30m & GP & 0.060726 & 0.168523 & 0.139771 & 0.337045 & 0.650602 \\
GE & Ind & 30m & SVR & / & / & / & 0.333019 & 0.604333 \\
GE & Ind & 30m & TimesFM & / & / & / & \underline{0.123975} & \underline{0.356935} \\
GE & Ind & 30m & TimeGPT & / & / & / & 0.425805 & 0.652852 \\
GE & Ind & 30m & Chronos-small & \underline{0.048455} & \underline{0.131499} & 0.129607 & 0.262997 & 0.559318 \\
GE & Ind & 30m & Moment & / & / & / & 0.524149 & 0.796408 \\
GE & Ind & 30m & Chronos-tiny & 0.049684 & 0.132013 & \underline{0.128836} & 0.264026 & 0.549092 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : GE-I-60}} \\
\hline

GE & Ind & 60m & Lag-llama & 0.152211 & 0.510377 & 0.507056 & 1.020754 & 1.730388 \\
GE & Ind & 60m & GP & 0.122323 & 0.337323 & 0.278522 & 0.674646 & 1.276264 \\
GE & Ind & 60m & SVR & / & / & / & 0.616670 & 1.180045 \\
GE & Ind & 60m & TimesFM & / & / & / & \underline{0.179344} & \underline{0.594087} \\
GE & Ind & 60m & TimeGPT & / & / & / & 0.504388 & 0.907498 \\
GE & Ind & 60m & Chronos-small & \underline{0.091911} & \underline{0.209760} & \underline{0.162205} & 0.419520 & 0.914137 \\
\hline
\textbf{Country} & \textbf{Type} & \textbf{Resolution} & \textbf{Model} & \textbf{Q 10\%} & \textbf{Q 50\%} & \textbf{Q 90\%} &\textbf{ MAE} & \textbf{RMSE} \\
\hline

GE & Ind & 60m & Moment & / & / & / & 1.019896 & 1.552359 \\
GE & Ind & 60m & Chronos-tiny & 0.104049 & 0.225248 & 0.176816 & 0.450496 & 0.958627 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : NL-A-60}} \\
\hline

NL & Agg & 60m & Lag-llama & 0.843935 & 1.852178 & 1.727107 & 3.704356 & 4.861644 \\
NL & Agg & 60m & GP & 0.291548 & 0.646336 & 0.306596 & 1.292672 & 1.806295 \\
NL & Agg & 60m & SVR & / & / & / & 1.472345 & 2.044546 \\
NL & Agg & 60m & TimesFM & / & / & / & \underline{1.009053} & 1.567828 \\
NL & Agg & 60m & TimeGPT & / & / & / & 1.053222 & \underline{1.466654} \\
NL & Agg & 60m & Chronos-small & 0.249438 & \underline{0.537236} & \underline{0.440845} & 1.074473 & 1.598724 \\
NL & Agg & 60m & Moment & / & / & / & 2.738191 & 3.459535 \\
NL & Agg & 60m & Chronos-tiny & \underline{0.240765} & 0.545286 & 0.456865 & 1.090573 & 1.616636 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : NL-I-60}} \\
\hline

NL & Ind & 60m & Lag-llama & 0.042126 & 0.117181 & 0.139105 & 0.234361 & 0.395725 \\
NL & Ind & 60m & GP & 0.041526 & 0.098189 & \underline{0.068128} & 0.196377 & 0.326855 \\
NL & Ind & 60m & SVR & / & / & / & 0.243757 & 0.307543 \\
NL & Ind & 60m & TimesFM & / & / & / & \underline{0.006106} & \underline{0.058067} \\
NL & Ind & 60m & TimeGPT & / & / & / & 0.154807 & 0.234427 \\
NL & Ind & 60m & Chronos-small & 0.022166 & \underline{0.071565} & 0.072857 & 0.143129 & 0.284994 \\
NL & Ind & 60m & Moment & / & / & / & 0.264652 & 0.366368 \\
NL & Ind & 60m & Chronos-tiny & \underline{0.021725} & 0.075490 & 0.083617 & 0.150981 & 0.299418 \\

% \bottomrule
% \endlastfoot
% Country & Type & Resolution & Model & Quantile 10\% & Quantile 50\% & Quantile 90\% & MAE & RMSE \\

\hline
\multicolumn{9}{c}{\textit{Experiment ID : UK-A-30}} \\
\hline
UK & Agg & 30m & Lag-llama & 0.045018 & 0.119832 & 0.135259 & 0.239664 & 0.451349 \\
UK & Agg & 30m & GP & 0.209277 & 0.088265 & 0.240850 & 0.176531 & 0.341280 \\
UK & Agg & 30m & SVR & / & / & / & 0.241066 & 0.338751 \\
UK & Agg & 30m & TimesFM & / & / & / & \underline{0.025922} & \underline{0.090576} \\
UK & Agg & 30m & TimeGPT & / & / & / & 0.153145 & 0.255350 \\
UK & Agg & 30m & Chronos-small & \underline{0.020027} & \underline{0.063683} & \underline{0.079859} & 0.127367 & 0.275875 \\
UK & Agg & 30m & Moment & / & / & / & 0.227259 & 0.363231 \\
UK & Agg & 30m & Chronos-tiny & 0.020914 & 0.065335 & 0.082447 & 0.130670 & 0.283750 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : UK-A-60}} \\
\hline

UK & Agg & 60m & Lag-llama & 0.038587 & 0.113048 & 0.123332 & 0.226096 & 0.405490 \\
UK & Agg & 60m & GP & 0.046247 & 0.105628 & 0.098074 & 0.211257 & 0.408938 \\
UK & Agg & 60m & SVR & / & / & / & 0.267612 & 0.404632 \\
UK & Agg & 60m & TimesFM & / & / & / & \underline{0.038940} & \underline{0.160942} \\
UK & Agg & 60m & TimeGPT & / & / & / & 0.170762 & 0.295124 \\
UK & Agg & 60m & Chronos-small & 0.022803 & 0.072750 & \underline{0.084599} & 0.145500 & 0.332297 \\
UK & Agg & 60m & Moment & / & / & / & 0.230894 & 0.386173 \\
UK & Agg & 60m & Chronos-tiny & \underline{0.022260} & \underline{0.072748} & 0.086059 & 0.145496 & 0.329293 \\
UK & Agg & 60m & Lag-llama & 0.050252 & 0.1323619 & 0.142208 & 0.264723 & 0.507108 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : UK-I-30}} \\
\hline

UK & Ind & 30m & Lag-llama & 0.036119 & 0.089907 & 0.095555 & 0.179814 & 0.334474 \\
UK & Ind & 30m & GP & 0.107600 & 0.084011 & 0.135837 & 0.168023 & 0.315311 \\
UK & Ind & 30m & SVR & / & / & / & 0.217501 & 0.299059 \\
UK & Ind & 30m & TimesFM & / & / & / & \underline{0.008541} & \underline{0.051992} \\
UK & Ind & 30m & TimeGPT & / & / & / & 0.135581 & 0.224905 \\
UK & Ind & 30m & Chronos-small & \underline{0.019020} & \underline{0.056365} & \underline{0.065028} & 0.112731 & 0.239053 \\
UK & Ind & 30m & Moment & / & / & / & 0.186289 & 0.291365 \\
UK & Ind & 30m & Chronos-tiny & 0.020274 & 0.057286 & 0.067766 & 0.114572 & 0.244053 \\
\hline
\multicolumn{9}{c}{\textit{Experiment ID : UK-I-60}} \\
\hline

UK & Ind & 60m & Lag-llama & 0.050252 & 0.132362 & 0.142209 & 0.264724 & 0.507108 \\
UK & Ind & 60m & GP & 0.054652 & 0.118893 & 0.102130 & 0.237786 & 0.437856 \\
UK & Ind & 60m & SVR & / & / & / & 0.269159 & 0.415563 \\
UK & Ind & 60m & TimesFM & / & / & / & \underline{0.012980} & \underline{0.092920} \\
\hline
\textbf{Country} & \textbf{Type} & \textbf{Resolution} & \textbf{Model} & \textbf{Q 10\%} & \textbf{Q 50\%} & \textbf{Q 90\%} &\textbf{ MAE} & \textbf{RMSE} \\
\hline

UK & Ind & 60m & TimeGPT & / & / & / & 0.181900 & 0.315460 \\
UK & Ind & 60m & Chronos-small & 0.023683 & \underline{0.074465} & \underline{0.086257} & 0.148930 & 0.335712 \\
UK & Ind & 60m & Moment & / & / & / & 0.267322 & 0.432852 \\
UK & Ind & 60m & Chronos-tiny & \underline{0.023578} & 0.075748 & 0.088633 & 0.151497 & 0.340863 \\
\hline
\label{exp_results}
\end{longtable}
\twocolumn
